SA-Attack: Improving Adversarial Transferability of Vision-Language Pre-training Models via Self-Augmentation

Current Visual-Language Pre-training (VLP) models are vulnerable to adversarial examples. These adversarial examples present substantial security risks to VLP models, as they can leverage inherent weaknesses in the models, resulting in incorrect predictions. In contrast to white-box adversarial attacks, transfer attacks (where the adversary crafts adversarial examples on a white-box model to fool another black-box model) are more reflective of real-world scenarios, thus making them more meaningful for research. By summarizing and analyzing existing research, we identified two factors that can influence the efficacy of transfer attacks on VLP models: inter-modal interaction and data diversity. Based on these insights, we propose a self-augment-based transfer attack method, termed SA-Attack. Specifically, during the generation of adversarial images and adversarial texts, we apply different data augmentation methods to the image modality and text modality, respectively, with the aim of improving the adversarial transferability of the generated adversarial images and texts. Experiments conducted on the FLickr30K and COCO datasets have validated the effectiveness of our method. Our code will be available after this paper is accepted.

==> tex/ack.tex <==
% use section* for acknowledgment
\ifCLASSOPTIONcompsoc
  % The Computer Society usually uses the plural form
  \section*{Acknowledgments}
\else
  % regular IEEE prefers the singular form
  \section*{Acknowledgment}
\fi


The authors would like to thank...

==> tex/pre.tex <==
\section{Discussions of Existing Attack Methods}



% In this section, we primarily discuss the limitations of existing adversarial attack methods on the VLP model, namely Sep-Attack \cite{zhang2022towards}, Co-Attack \cite{zhang2022towards}, and SGA \cite{lu2023set}, in terms of adversarial transferability. Figure \ref{fig_com} provides a comparison of these methods.

% \noindent \textbf{Sep-Attack} ignores the interaction between image and text modality. Existing research \cite{zhou2023advclip} points out that there has a gap between image modality and text modality. When designing attack methods for the VLP models, which includes both text and image modalities, neglecting this gap could potentially impact the adversarial transferability.

% \noindent \textbf{Co-Attack} does not take into account the diversity between image-text pairs. Although compared to Sep-Attack, Co-Attack considers the interaction between multi-modalities. However, Co-Attack only uses one image-text pair to craft adversarial examples. Many studies \cite{wang2023structure,byun2022improving,wang2021admix} have shown that the diversity of input data is one of the important factors affecting adversarial transferability.

% \noindent \textbf{SGA} employs a limited diversity between image-text pairs. Compared to the first two attack methods, SGA not only considers the interaction between multi-modalities, but also takes into account the diversity of input data. However, SGA only considers the scale-invariance in images. The diversity of text modality, as well as other properties of image modalities (such as translation invariance, structural invariance), have not yet been considered.

% The above analysis motivates us to improve existing methods from the perspective of data diversity.
